Custom Tailored Suite of Random Forests for Prefetcher Adaptation

To close the gap between memory and processors, and in turn improve performance, there has been an abundance of work in the area of data/instruction prefetcher designs. Prefetchers are deployed in each level of the memory hierarchy, but typically, each prefetcher gets designed without comprehensively accounting for other prefetchers in the system. As a result, these individual prefetcher designs do not always complement each other, and that leads to low average performance gains and/or many negative outliers. In this work, we propose SuitAP (Suite of random forests for Adaptation of Prefetcher system configuration), which is a hardware prefetcher adapter that uses a suite of random forests to determine at runtime which prefetcher should be ON at each memory level, such that they complement each other. Compared to a design with no prefetchers, using SuitAP we improve IPC by 46% on average across traces generated from SPEC2017 suite with 12KB overhead. Moreover, we also reduce negative outliers using SuitAP.

==> definitions.tex <==

\section{Definitions}
\label{sec:defines}
In this section we define various terms used throughout this paper.\break
%
$\bullet$ \textbf{Prefetcher System Configuration (PSC) -} {\color{red}A PSC specifies
which prefetcher is selected at each level of the memory in the system.} \ignore{For example, {\color{red}if there are
two prefetchers at L1D\$, $L1D\$_{PF1}$ and $L1D\$_{PF2}$, and two prefetchers at L2\$, $L2\$_{PF1}$ and $L2\$_{PF2}$,  in a processor, then there are nine possible
PSCs -- \{$L1D\$_{PF1}$=ON, $L1D\$_{PF2}$=ON, $L1D\$_{PF1,2}$=OFF\} $\times$ \{$L2\$_{PF1}$=ON, $L2\$_{PF2}$=ON, $L2\$_{PF1,2}$=OFF\}. For a system with $N_{pf}$ prefetchers at 4 memory levels, there are
$N_{psc}=(N_{pf}+1)^4$ possible PSCs.}} \break
%
$\bullet$ \textbf{Class -} Each PSC has an associated class and classifier.
\break
%
$\bullet$ \textbf{{\color{black}Events Per Thousand Instructions (E-PTI)} -}
E-PTI corresponds to the average number of occurrences of a hardware event per 
thousand instructions. We use these values as the features of our ML model. {\ignore{\color{black} We use hardware performance
counters (HPCs) to count the number of occurrences of various hardware-level
events in a processor. We then calculate the E-PTI value from these events, and use
those calculated values as the features of our ML model.}} %\break
\ignore{
\begin{table*}[h]
  \caption{\textbf{Comparison with prior work -} {We compare \myalgo~with prior
  work on prefetcher adapters. We use \textit{NA}
  when \color{black}the paper lacks information about the respective metric. In the last column, for the papers that do not approach the problem from the hardware perspective we state ``Software''. }}
  \label{tab:prior}
\scriptsize
\renewcommand{\arraystretch}{1.0}
\centering
\begin{tabular}{P{1.2cm}|P{1.5cm}|P{2.5cm}|P{3.05cm}|P{3.8cm}|P{1.6cm}|P{1.1cm}}
\hline
\textbf{Work} & \textbf{\# Prefetchers} & \textbf{IPC
Gain Over Baseline PSC} & \textbf{Baseline PSC IPC Gain Over No Prefetching} &
\textbf{Dataset}
&
\textbf{Heuristic or Data-Driven} & \textbf{Overhead} \\
\hline
\hline
\cite{liao2009machine} & 4 prefetchers & Max: \textit{NA}, Avg: \textit{NA} & \textit{NA} & SPEC
CPU\textsuperscript \textregistered~2006 + 11 Datacenter  & Data-Driven & Software \\
\hline
\cite{zeng2017long} & 1 prefetcher & Max: \textit{NA}, Avg: \textit{NA} & \textit{NA} & 6 synthetic \trace s   & Data-Driven & $\sim15$KB \\
\hline
\cite{bhatia2019perceptron} & 1 prefetcher & Max: 10\%, Avg: 2.27\%  &
15.24\% & SPEC CPU\textsuperscript \textregistered~2017 & Data-Driven & $\sim39$KB\\
\hline
\cite{hiebel2019machine} & 4 prefetchers & Max: 15\% to 20\%, Avg: -1\% to 3.6\% & -1\% to 8.5\% \ignore{(with one prefetcher disabled)} &
Memory-intensive Apps from SPEC CPU\textsuperscript \textregistered and
PARSEC \cite{bienia2008parsec} & Data-Driven &
Software\\
\hline
\cite{jimenez2012making}~ & 1 prefetcher & Max: $2.7\times$,
Avg: \textit{NA} & \textit{NA} & SPEC CPU\textsuperscript
\textregistered~2006 & Heuristic-Based & Software\\
\hline
\cite{rahman2015maximizing}~  & 4 prefetchers & Max: $1.4\times$,
Avg: \textit{NA} &\textit{NA} & PARSEC \cite{bienia2008parsec} & Data-Driven &  Software \\
\hline
\cite{kang2013hardware}~  & 0 prefetchers & Max: 20\%, Avg: 11\% & Same & PARSEC \cite{bienia2008parsec}& Heuristic-base &  Software \\
\hline
\myalgo~ & 6 prefetchers & Max: 28\%, Avg: 5\% & $>50$\% & 132 Apps from 6 Data Suites &
Data-Driven & $\sim10$KB\\
\hline
\end{tabular}
  \vspace{-0.2in}
\end{table*} \break
$\bullet$ \textbf{\trace~-} A \trace~is a group of instructions that represent a
particular behavior. One or more \trace s can be used to represent the behavior
of a benchmark. For example, a benchmark with consistent looping behavior can be
represented by one \trace~corresponding to a single iteration of the loop. We construct one or
more unique representative \trace s from each benchmark
\cite{perelman2003picking}. In total, we construct 2051 \trace s.
}
%
\break
$\bullet$ \textbf{Instruction Window -} An instruction window is a set of
instructions. At runtime, at the end of every instruction window, we calculate
the E-PTIs and use them as input to our ML model, which predicts the best PSC
 \ignore{In this work we experimented with different
window sizes and did not see a large change in the performance of \myalgo. We
set the instruction window size to 1,000,000 instructions.}\break
%
\ignore{$\bullet$ \textbf{Dataset -} To generate our dataset, we run each \trace~with
each PSC i.e., we do $185$ \trace s * $N_{psc}$ different runs. For each run, we
determine the average E-PTI values and the IPC value {\color{red}every 1,000,000 instructions. We run each trace for 100,000,000 instructions. We
construct the dataset consisting of E-PTI values as features and the IPC values
as labels. More details are provided in subsubsection \ref{sec:training_details}}}
\ignore{$\bullet$ \textbf{Baseline PSC -} This is the default PSC that we
see in real systems today. Here all prefetchers are ON and they are
controlled by the native control policies at runtime. More details are provided in
Section \ref{sec:suitap_overview}.} 
%backup for table
\ignore{
\begin{table*}[h]
  \caption{\textbf{Comparison with prior work -} {We compare \myalgo~with prior
  work on prefetcher adapters using a variety of metrics. We use \textit{NA}
  when \color{black}the paper lacks information about the respective metric. In
  the Overhead column, for the papers that use software prefetchers, the
  overhead is not provided and so we just state ``Software''. }}
  \label{tab:prior}
\scriptsize
\renewcommand{\arraystretch}{1.0}
\centering
\begin{tabular}{P{1.2cm}|P{1.5cm}|P{2.5cm}|P{2.05cm}|P{3.8cm}|P{1.6cm}|P{2cm}|P{1.1cm}}
\hline
\textbf{Work} & \textbf{\# Prefetchers} & \textbf{IPC
Gain Over Baseline PSC} & \textbf{IPC Gain Over No Prefetching} &
\textbf{Dataset}
&
\textbf{Heuristic or Data-Driven} & \textbf{Complexity or
Adaptation}& \textbf{Overhead} \\
\hline
\hline
\cite{liao2009machine} & 4 prefetchers & Max:\missingcitation, Avg: 1.33\% & \textit{NA} & SPEC
CPU\textsuperscript \textregistered~2006 + 11 Datacenter  & Data-Driven &
Insights
from Data & Software \\
\hline
\cite{bhatia2019perceptron} & 1 prefetcher & Max:\missingcitation, Avg: 2.27\%  &
Max:\missingcitation, Avg: 15.24\% & SPEC CPU\textsuperscript \textregistered~2017 & Data-Driven & More
Complex Prefetcher Design & $\sim39$KB\\
\hline
\cite{hiebel2019machine} & 4 prefetchers & Max:\missingcitation, Avg: -1\% to 5\% & \textit{NA} &
Memory-intensive Apps from SPEC CPU\textsuperscript \textregistered~2006 and
PARSEC \cite{bienia2008parsec} & Data-Driven & Highly Dependent on Dataset&
Software\\
\hline
\cite{jimenez2012making}~ & 1 prefetcher & Max: $2.7\times$,
Avg: \textit{NA} & \textit{NA} & SPEC CPU\textsuperscript
\textregistered~2006 & Heuristic-Based & Insights
from Data & Software\\
\hline
\cite{rahman2015maximizing}~  & 4 prefetchers & Max: $1.4\times$,
Avg: \textit{NA} &\textit{NA} & PARSEC \cite{bienia2008parsec} & Data-Driven &
Insights
from Data &  Software \\
\hline
\cite{kang2013hardware}~  & 0 prefetchers & Max: 20\%, Avg: 11\% & Same & PARSEC \cite{bienia2008parsec}& Heuristic-based & Insights
from Data
 &  Software \\
\hline
\myalgo~ & 6 prefetchers & Max: 28\%, Avg: 5\% & $>50$\% & 132 Apps from 6 Data Suites &
Data-Driven & Adaptation Scheme & $\sim10$KB\\
\hline
\end{tabular}
  \vspace{-0.3in}
\end{table*}
}

==> discussion.tex <==
\section{Future Work}

In this work, we apply auto-optimization to constructed tree pruning. We can
also provide
additional auto-optimization options. Each tree could
choose the classes used for training pruning threshold instead of using the same
pruning threshold. This additional specialization would create a substantially
larger solution space and would require us to use search algorithms instead of
exhaustive search.

\ignore{For multiple outputs, we have only considered the most straightforward
selection mechanism, dividing each instruction window evenly for each output.
With a better selection mechanism, we can further reduce the hardware overhead
and increase IPC.}

We plan to create a
many-core version of \myalgo~with some control mechanism between each of the
cores. The complex interactions between prefetchers on-core is amplified when
there are multiple cores in the system. This requires \myalgo~to support a more
complicated scheme for arbitrating local \myalgo~decisions across different
cores. For many-threads, a single \myalgo~needs to be carefully trained to
handle multiple benchmarks running at the same time. \ignore{Enabling multi-core
\myalgo~would further increase the IPC since each core would be able to adapt to
their unique conditions.}


==> outline.tex <==

\section{Outline}
\begin{itemize}
    \item Introduction 
    \begin{itemize}
        \item Memory wall problem.
        \item Prefetching as a solution.
        \item Prefetchers designed in isolation and negative outliers problem. TODO: Need to reword the introduction and the problems to focus more on negative outliers.
        \item Our solution is by using ML and designing a hardware adaptor.
        \item {\color{red}TODO: Will we add a motivation figure?}
        \item {\color{red}Will add discussion on invariance and how that is a contribution.}
    \end{itemize}
    \item Definitions
    \begin{itemize}
        \item PSC.
        \item Class. {\color{red}TODO: We are actually getting better results with regression-based approach. I need to decide on if to leave this for HPCA or include this here.}
        \item E-PTI.
        \item Simpoints or traces.
        \item Instruction window.
        \item Dataset. {\color{red}TODO: This will now be for quant not for whole simpoint, instruction window and simpoint sample have esentially merged into the dataset. We now have quants.}
        \item Baseline PSC: {\color{red} The baseline is now not all the prefetchers being turned ON. It is rather the setting that we observed to have the greatest coverage.}
        \item {\color{red}TODO: Add invariance.}
    \end{itemize}
    \item Related Work: \begin{itemize}
        \item Can stay largely the same but we need to remove emphasis on overheads (since the comparison will be largely not in our favor. 
        \item The table might be removed altogether. Since the dataset is also not the focus anymore.
    \end{itemize}
    \item Suitap Design
    \begin{itemize}
        \item Suitap System Overview
        \begin{itemize}
            \item Figure with system overview.
            \item Discussion regarding the way suitap interacts with the prefetching system. {\color{red} TODO: change tone a little bit to state that the system uses a single prefetcher at a time. Reduce emphasis on heuristic control because that doesn't exist anymore in this system}
            \item {\color{red}Without the heuristic control policy emphasis this section might actually collapse into the hardware section. It doesn't give much extra information.}
        \end{itemize}
        \item Suitap Algorithm:
        \begin{itemize}
        \item Multi-label vs Binary {\color{red} This will change if we go for the regression route. The other option is to save it for HPCA.}
        \item Table with different class preferences for each trace.
        \item Suite of Trees vs. Monolithic Tree. {\color{red} Will be updated to be suite of random forests vs monolithic tree}.
        \item Figure comparing Suitap with monolithic. {\color{red} Update to random forest instead of trees.}
        \item Suite of random forests vs NN.
        \item Training Suitap {\color{red} Discussion regarding invariance and the next quant prediction will be added here.}
        \item {\color{red}Choosing our classes discussion. How we pruned the number of classes down to 12 from 120.}
        \end{itemize}
        \item Suitap Hardware Design.
        \begin{itemize}
            \item Suitap Microarch design.
            \item Figure with suitap hardware. {\color{red} Update to reflect the random forests instead of just singular trees.}
            \item Overfitting discussion and how we handle this with quant construction + pruning + low amount of data used for training. 
            \item Table with features. {\color{red} Will need to update with the new features.}
            \item Optimization and pruning. {\color{red} This section might be removed because of space. Converge it into the overfitting and have a single sentence. We no longer have classes for training pruning so that only leaves two.}
        \end{itemize}
    \end{itemize}
    \item Evaluation
    \begin{itemize}
        \item Methodology:
        \begin{itemize} 
        \item Explain champsim modifications, architecture, prefetchers used at each level, SPEC2017. 
        \item Maybe a table for the architecture.
        \item Evaluation results
        \end{itemize}
        \begin{itemize}
            \item Suite vs Monolithic. {\color{red}Will we have this comparison? If so I can run experiments for it.}
            \item Main plot with comparison with prefetching competitions 1st and 3rd. This figure will now be long and probably double row instead of half a column. 
            \item Varibility study in number of nodes, estimators, and data training size (or leave it for HPCA).
        \end{itemize}
        \item Conclusion Future work.
    \end{itemize}
\end{itemize}
